The Sloan Digital Sky Survey extended point spread functions

A robust and extended characterization of the point spread function (PSF) is crucial to extract the photometric information produced by deep imaging surveys. Here, we present the extended PSFs of the Sloan Digital Sky Survey (SDSS), one of the most productive astronomical surveys of all time. By stacking ~1000 images of individual stars with different brightness, we obtain the bidimensional SDSS PSFs extending over 8 arcmin in radius for all the SDSS filters(u, g, r, i, z). This new characterization of the SDSS PSFs is near a factor of 10 larger in extension than previous PSFs characterizations of the same survey. We found asymmetries in the shape of the PSFs caused by the drift scanning observing mode. The flux of the PSFs is larger along the drift scanning direction. Finally, we illustrate with an example how the PSF models can be used to remove the scattered light field produced by the brightest stars in the central region of the Coma cluster field. This particular example shows the huge importance of PSFs in the study of the low-surface brightness Universe, especially with the upcoming of ultradeep surveys, such as the Large Synoptic Survey Telescope (LSST). Following a reproducible science philosophy, we make all the PSF models and the scripts used to do the analysis of this paper publicly available (snapshot v0.5-0-g62d83df).

==> reproduce/analysis/bash/download-multi-try <==
#!/bin/bash
#
# Attempt downloading multiple times before crashing whole project. From
# the top project directory (for the shebang above), this script must be
# run like this:
#
#   $ /path/to/download-multi-try downloader lockfile input-url downloaded-name
#
# NOTE: The `downloader' must contain the option to specify the output name
# in its end. For example "wget -O". Any other option can also be placed in
# the middle.
#
# Due to temporary network problems, a download may fail suddenly, but
# succeed in a second try a few seconds later. Without this script that
# temporary glitch in the network will permanently crash the project and
# it can't continue. The job of this script is to be patient and try the
# download multiple times before crashing the whole project.
#
# LOCK FILE: Since there is usually only one network port to the outside
# world, downloading is done much faster in serial, not in parallel. But
# the project's processing may be done in parallel (with multiple threads
# needing to download different files at the same time). Therefore, this
# script uses the `flock' program to only do one download at a time. To
# benefit from it, any call to this script must be given the same lock
# file. If your system has multiple ports to the internet, or for any
# reason, you don't want to use a lock file, set the `lockfile' name to
# `nolock'.
#
# Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This script is free software: you can redistribute it and/or modify it
# under the terms of the GNU General Public License as published by the
# Free Software Foundation, either version 3 of the License, or (at your
# option) any later version.
#
# This script is distributed in the hope that it will be useful, but
# WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the GNU General
# Public License for more details. See <http://www.gnu.org/licenses/>.





# Script settings
# ---------------
# Stop the script if there are any errors.
set -e





# Input arguments and necessary sanity checks.
inurl="$3"
outname="$4"
lockfile="$2"
downloader="$1"
if [ "x$downloader" = x ]; then
    echo "$0: downloader (first argument) not given."; exit 1;
fi
if [ "x$lockfile" = x ]; then
    echo "$0: lock file (second argument) not given."; exit 1;
fi
if [ "x$inurl" = x ]; then
    echo "$0: full input URL (third argument) not given."; exit 1;
fi
if [ "x$outname" = x ]; then
    echo "$0: output name (fourth argument) not given."; exit 1;
fi





# Try downloading multiple times before crashing.
counter=0
maxcounter=10
while [ ! -f "$outname" ]; do

    # Increment the counter. We need the `counter=' part here because
    # without it the evaluation of arithmetic expression will be like and
    # error and the script is set to crash on errors.
    counter=$((counter+1))

    # If we have passed a maximum number of trials, just exit with
    # a failed code.
    if (( counter > maxcounter )); then
        echo
	echo "Failed $maxcounter download attempts: $outname"
        echo
	exit 1
    fi

    # If this isn't the first attempt print a notice and wait a little for
    # the next trail.
    if (( counter > 1 )); then
	tstep=$((counter*5))
        echo "Download trial $counter for '$outname' in $tstep seconds."
        sleep $tstep
    fi

    # Attempt downloading the file (one-at-a-time). Note that the
    # `downloader' ends with the respective option to specify the output
    # name. For example "wget -O" (so `outname', that comes after it) will
    # be the name of the downloaded file.
    if [ x"$lockfile" = xnolock ]; then
        if ! $downloader $outname $inurl; then rm -f $outname; fi
    else
        flock "$lockfile" bash -c \
              "if ! $downloader $outname $inurl; then rm -f $outname; fi"
    fi

done





# Return successfully
exit 0


==> reproduce/software/bash/git-post-checkout <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the `metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# This script is taken from the `examples/hooks/pre-commit' file of the
# `metastore' package (installed within the project, with an MIT license
# for copyright). We have just changed the name of the `MSFILE' and also
# set special characters for the installation location of meta-store so our
# own installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.


# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Delete all temporary files
find @TOP_PROJECT_DIR@/ -name "*~" -type f -delete

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Run metastore.
exit_on_fail \
       $MSBIN -a -m -e -E -q -O @USER@ -G @GROUP@ -f "$MSFILE"

# Return with a success code (0).
exit 0


==> reproduce/software/bash/git-pre-commit <==
#!@BINDIR@/bash
#
# The example hook script to store the metadata information of version
# controlled files (with each commit) using the `metastore' program.
#
# Copyright (C) 2016 Przemyslaw Pawelczyk <przemoc@gmail.com>
# Copyright (C) 2018-2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
#
# WARNING:
#
# If the commit is aborted (e.g. by not entering any synopsis),
# then updated metastore file (.metadata by default) is not reverted,
# so its new version remains in the index.
# To undo any changes in metastore file written since HEAD commit,
# you may want to reset and checkout HEAD version of the file:
#
#     git reset HEAD -- .metadata
#     git checkout HEAD -- .metadata
#
# This script is taken from the `examples/hooks/pre-commit' file of the
# `metastore' package (installed within the project, with an MIT license
# for copyright). Here, the name of the `MSFILE' and also set special
# characters for the installation location of meta-store so our own
# installation is found by Git.
#
# Permission is hereby granted, free of charge, to any person obtaining a
# copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to permit
# persons to whom the Software is furnished to do so, subject to the
# following conditions:
#
# The above copyright notice and this permission notice shall be included
# in all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS
# OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT. IN
# NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY CLAIM,
# DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT, TORT OR
# OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE
# USE OR OTHER DEALINGS IN THE SOFTWARE.

# File containig the metadata and metastore executable.
MSFILE=".file-metadata"
MSBIN=@BINDIR@/metastore

# If metastore is not installed, then ignore this script (exit with a
# status of 0).
if [ ! -f $MSBIN ]; then exit 0; fi

# Function to help in reporting a crash.
exit_on_fail() {
	"$@"
	if [ $? -ne 0 ]; then
		echo "Failed to execute: $@" >&2
		exit 1
	fi
}

# Run metastore.
exit_on_fail \
	$MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"

# If it's first metastore commit, store again to include $MSFILE in $MSFILE.
if ! git-ls-tree --name-only HEAD 2>/dev/null | grep -Fqx "$MSFILE"; then
	exit_on_fail \
	        $MSBIN -O @USER@ -G @GROUP@ -s -f "$MSFILE"
fi

# Check if the metadata file exists.
if [ ! -e "$MSFILE" ]; then
	echo "\"$MSFILE\" missing" >&2
	exit 1
fi

# Add the metadata file to the Git repository.
exit_on_fail \
	git-add "$MSFILE"

# Return with a success code (0).
exit 0


==> reproduce/software/bibtex/astrometrynet.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astrometrynet,
	doi = {10.1088/0004-6256/139/5/1782},
	url = {https://doi.org/10.1088%2F0004-6256%2F139%2F5%2F1782},
	year = 2010,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {139},
	number = {5},
	pages = {1782},
	author = {Dustin Lang and David W. Hogg and Keir Mierle and Michael Blanton and Sam Roweis},
	title = {{ASTROMETRY}.{NET}: {BLIND} {ASTROMETRIC} {CALIBRATION} {OF} {ARBITRARY} {ASTRONOMICAL} {IMAGES}},
	journal = {AJ}
}


==> reproduce/software/bibtex/astropy.tex <==
%% Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{astropy2018,
   author = {{Astropy Collaboration} and {Price-Whelan}, A.~M. and {Sip{\H o}cz}, B.~M. and
	{G{\"u}nther}, H.~M. and {Lim}, P.~L. and {Crawford}, S.~M. and
	{Conseil}, S. and {Shupe}, D.~L. and {Craig}, M.~W. and {Dencheva}, N. and
	{Ginsburg}, A. and {VanderPlas}, J.~T. and {Bradley}, L.~D. and
	{P{\'e}rez-Su{\'a}rez}, D. and {de Val-Borro}, M. and {Aldcroft}, T.~L. and
	{Cruz}, K.~L. and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Ardelean}, C. and {Babej}, T. and {Bach}, Y.~P. and {Bachetti}, M. and
	{Bakanov}, A.~V. and {Bamford}, S.~P. and {Barentsen}, G. and
	{Barmby}, P. and {Baumbach}, A. and {Berry}, K.~L. and {Biscani}, F. and
	{Boquien}, M. and {Bostroem}, K.~A. and {Bouma}, L.~G. and {Brammer}, G.~B. and
	{Bray}, E.~M. and {Breytenbach}, H. and {Buddelmeijer}, H. and
	{Burke}, D.~J. and {Calderone}, G. and {Cano Rodr{\'{\i}}guez}, J.~L. and
	{Cara}, M. and {Cardoso}, J.~V.~M. and {Cheedella}, S. and {Copin}, Y. and
	{Corrales}, L. and {Crichton}, D. and {D'Avella}, D. and {Deil}, C. and
	{Depagne}, {\'E}. and {Dietrich}, J.~P. and {Donath}, A. and
	{Droettboom}, M. and {Earl}, N. and {Erben}, T. and {Fabbro}, S. and
	{Ferreira}, L.~A. and {Finethy}, T. and {Fox}, R.~T. and {Garrison}, L.~H. and
	{Gibbons}, S.~L.~J. and {Goldstein}, D.~A. and {Gommers}, R. and
	{Greco}, J.~P. and {Greenfield}, P. and {Groener}, A.~M. and
	{Grollier}, F. and {Hagen}, A. and {Hirst}, P. and {Homeier}, D. and
	{Horton}, A.~J. and {Hosseinzadeh}, G. and {Hu}, L. and {Hunkeler}, J.~S. and
	{Ivezi{\'c}}, {\v Z}. and {Jain}, A. and {Jenness}, T. and {Kanarek}, G. and
	{Kendrew}, S. and {Kern}, N.~S. and {Kerzendorf}, W.~E. and
	{Khvalko}, A. and {King}, J. and {Kirkby}, D. and {Kulkarni}, A.~M. and
	{Kumar}, A. and {Lee}, A. and {Lenz}, D. and {Littlefair}, S.~P. and
	{Ma}, Z. and {Macleod}, D.~M. and {Mastropietro}, M. and {McCully}, C. and
	{Montagnac}, S. and {Morris}, B.~M. and {Mueller}, M. and {Mumford}, S.~J. and
	{Muna}, D. and {Murphy}, N.~A. and {Nelson}, S. and {Nguyen}, G.~H. and
	{Ninan}, J.~P. and {N{\"o}the}, M. and {Ogaz}, S. and {Oh}, S. and
	{Parejko}, J.~K. and {Parley}, N. and {Pascual}, S. and {Patil}, R. and
	{Patil}, A.~A. and {Plunkett}, A.~L. and {Prochaska}, J.~X. and
	{Rastogi}, T. and {Reddy Janga}, V. and {Sabater}, J. and {Sakurikar}, P. and
	{Seifert}, M. and {Sherbert}, L.~E. and {Sherwood-Taylor}, H. and
	{Shih}, A.~Y. and {Sick}, J. and {Silbiger}, M.~T. and {Singanamalla}, S. and
	{Singer}, L.~P. and {Sladen}, P.~H. and {Sooley}, K.~A. and
	{Sornarajah}, S. and {Streicher}, O. and {Teuben}, P. and {Thomas}, S.~W. and
	{Tremblay}, G.~R. and {Turner}, J.~E.~H. and {Terr{\'o}n}, V. and
	{van Kerkwijk}, M.~H. and {de la Vega}, A. and {Watkins}, L.~L. and
	{Weaver}, B.~A. and {Whitmore}, J.~B. and {Woillez}, J. and
	{Zabalza}, V. and {Astropy Contributors}},
    title = "{The Astropy Project: Building an Open-science Project and Status of the v2.0 Core Package}",
  journal = {AJ},
archivePrefix = "arXiv",
   eprint = {1801.02634},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, methods: statistical, reference systems },
     year = 2018,
    month = sep,
   volume = 156,
      eid = {123},
    pages = {123},
      doi = {10.3847/1538-3881/aabc4f},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2018AJ....156..123A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{astropy2013,
   author = {{Astropy Collaboration} and {Robitaille}, T.~P. and {Tollerud}, E.~J. and
	{Greenfield}, P. and {Droettboom}, M. and {Bray}, E. and {Aldcroft}, T. and
	{Davis}, M. and {Ginsburg}, A. and {Price-Whelan}, A.~M. and
	{Kerzendorf}, W.~E. and {Conley}, A. and {Crighton}, N. and
	{Barbary}, K. and {Muna}, D. and {Ferguson}, H. and {Grollier}, F. and
	{Parikh}, M.~M. and {Nair}, P.~H. and {Unther}, H.~M. and {Deil}, C. and
	{Woillez}, J. and {Conseil}, S. and {Kramer}, R. and {Turner}, J.~E.~H. and
	{Singer}, L. and {Fox}, R. and {Weaver}, B.~A. and {Zabalza}, V. and
	{Edwards}, Z.~I. and {Azalee Bostroem}, K. and {Burke}, D.~J. and
	{Casey}, A.~R. and {Crawford}, S.~M. and {Dencheva}, N. and
	{Ely}, J. and {Jenness}, T. and {Labrie}, K. and {Lim}, P.~L. and
	{Pierfederici}, F. and {Pontzen}, A. and {Ptak}, A. and {Refsdal}, B. and
	{Servillat}, M. and {Streicher}, O.},
    title = "{Astropy: A community Python package for astronomy}",
  journal = {A\&A},
archivePrefix = "arXiv",
   eprint = {1307.6212},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, methods: miscellaneous, virtual observatory tools},
     year = 2013,
    month = oct,
   volume = 558,
      eid = {A33},
    pages = {A33},
      doi = {10.1051/0004-6361/201322068},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2013A\%26A...558A..33A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/corner.tex <==
%% Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{corner,
       author = {{Foreman-Mackey}, Daniel},
        title = "{corner.py: Scatterplot matrices in Python}",
      journal = {The Journal of Open Source Software},
         year = "2016",
        month = "Jun",
       volume = {1},
        pages = {24},
          doi = {10.21105/joss.00024},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016JOSS....1...24F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/cython.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{cython2011,
   author = {{Behnel}, S. and {Bradshaw}, R. and {Citro}, C. and {Dalcin}, L. and
	{Seljebotn}, D.~S. and {Smith}, K.},
    title = "{Cython: The Best of Both Worlds}",
  journal = {CiSE},
     year = 2011,
    month = mar,
   volume = 13,
   number = 2,
    pages = {31},
      doi = {10.1109/MCSE.2010.118},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2011CSE....13b..31B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/fftw.tex <==
%% Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{fftw,
   author = {M. {Frigo} and S. G. {Johnson}},
  journal = {IEEE Proc.},
    title = {The Design and Implementation of FFTW3},
     year = {2005},
   volume = {93},
   number = {2},
    pages = {216},
      doi = {10.1109/JPROC.2004.840301},
     ISSN = {0018-9219},
    month = {Feb},
}


==> reproduce/software/bibtex/galsim.tex <==
%% Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{galsim,
       author = {{Rowe}, B.~T.~P. and {Jarvis}, M. and {Mandelbaum}, R. and
         {Bernstein}, G.~M. and {Bosch}, J. and {Simet}, M. and {Meyers}, J.~E. and
         {Kacprzak}, T. and {Nakajima}, R. and {Zuntz}, J. and {Miyatake}, H. and
         {Dietrich}, J.~P. and {Armstrong}, R. and {Melchior}, P. and
         {Gill}, M.~S.~S.},
        title = "{GALSIM: The modular galaxy image simulation toolkit}",
      journal = {Astronomy and Computing},
     keywords = {Methods: data analysis, Techniques: image processing, Gravitational lensing, Cosmology: observations, Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics, 85-04},
         year = "2015",
        month = "Apr",
       volume = {10},
        pages = {121-150},
          doi = {10.1016/j.ascom.2015.02.002},
archivePrefix = {arXiv},
       eprint = {1407.7676},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&C....10..121R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/gnuastro.tex <==
%% Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{gnuastro,
   author = {{Akhlaghi}, M. and {Ichikawa}, T.},
    title = "{Noise-based Detection and Segmentation of Nebulous Objects}",
  journal = {ApJS},
archivePrefix = "arXiv",
   eprint = {1505.01664},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: irregular, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric},
     year = 2015,
    month = sep,
   volume = 220,
      eid = {1},
    pages = {1},
      doi = {10.1088/0067-0049/220/1/1},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2015ApJS..220....1A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/healpix.tex <==
@ARTICLE{healpix,
       author = {{G{\'o}rski}, K.~M. and {Hivon}, E. and {Banday}, A.~J. and {Wand
        elt}, B.~D. and {Hansen}, F.~K. and {Reinecke}, M. and {Bartelmann}, M.},
        title = "{HEALPix: A Framework for High-Resolution Discretization and Fast Analysis of Data Distributed on the Sphere}",
      journal = {ApJ},
     keywords = {Cosmology: Cosmic Microwave Background, Cosmology: Observations, Methods: Statistical, Astrophysics},
         year = "2005",
        month = "Apr",
       volume = {622},
       number = {2},
        pages = {759},
          doi = {10.1086/427976},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409513},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2005ApJ...622..759G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/imfit.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{imfit2015,
   author = {{Erwin}, P.},
    title = "{IMFIT: A Fast, Flexible New Program for Astronomical Image Fitting}",
  journal = {ApJ},
archivePrefix = "arXiv",
   eprint = {1408.1097},
 primaryClass = "astro-ph.IM",
 keywords = {galaxies: bulges, galaxies: photometry, galaxies: structure, methods: data analysis, techniques: image processing, techniques: photometric },
     year = 2015,
    month = feb,
   volume = 799,
      eid = {226},
    pages = {226},
      doi = {10.1088/0004-637X/799/2/226},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2015ApJ...799..226E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/matplotlib.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@Article{matplotlib2007,
  Author    = {Hunter, J. D.},
  Title     = {Matplotlib: A 2D graphics environment},
  Journal   = {CiSE},
  Volume    = {9},
  Number    = {3},
  Pages     = {90},
  abstract  = {Matplotlib is a 2D graphics package used for Python
  for application development, interactive scripting, and
  publication-quality image generation across user
  interfaces and operating systems.},
  publisher = {IEEE COMPUTER SOC},
  doi       = {10.1109/MCSE.2007.55},
  year      = 2007
}


==> reproduce/software/bibtex/mpi4py.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{mpi4py2011,
   author = {{Dalcin}, L.~D. and {Paz}, R.~R. and {Kler}, P.~A. and {Cosimo}, A.
	},
    title = "{Parallel distributed computing using Python}",
  journal = {Advances in Water Resources},
     year = 2011,
    month = sep,
   volume = 34,
    pages = {1124},
      doi = {10.1016/j.advwatres.2011.04.013},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2011AdWR...34.1124D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/numpy.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{numpy2011,
   author = {{van der Walt}, S. and {Colbert}, S.~C. and {Varoquaux}, G.},
    title = "{The NumPy Array: A Structure for Efficient Numerical Computation}",
  journal = {CiSE},
archivePrefix = "arXiv",
   eprint = {1102.1523},
 primaryClass = "cs.MS",
     year = 2011,
    month = mar,
   volume = 13,
   number = 2,
    pages = {22},
      doi = {10.1109/MCSE.2011.37},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2011CSE....13b..22V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/scamp.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scamp,
   author = {{Bertin}, E.},
    title = "{Automatic Astrometric and Photometric Calibration with SCAMP}",
     year = 2006,
   journal= {ASPConf},
   volume = 351,
    month = jul,
    pages = {112},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2006ASPC..351..112B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/scipy.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{scipy2011,
   author = {K. J. {Millman} and M. {Aivazis}},
  journal = {CiSE},
    title = {Python for Scientists and Engineers},
     year = {2011},
   volume = {13},
   number = {2},
    pages = {9},
 keywords = {Special issues and sections;Computer languages;Programming;Scientific computing;Numerical models;Programming languages;Python;Scientific computing;interactive research;Python libraries;Python tools},
      doi = {10.1109/MCSE.2011.36},
     ISSN = {1521-9615},
    month ={March},
}

@ARTICLE{scipy2007,
   author = {T. E. {Oliphant}},
  journal = {CiSE},
    title = {Python for Scientific Computing},
     year = {2007},
   volume = {9},
   number = {3},
    pages = {10},
 keywords = {high level languages;Python;scientific computing;steering language;scientific codes;high-level language;Scientific computing;High level languages;Libraries;Writing;Application software;Embedded software;Software standards;Standards development;Internet;Prototypes;Python;computer languages;scientific programming;scientific computing},
      doi = {10.1109/MCSE.2007.58},
     ISSN = {1521-9615},
    month = {May},
}


==> reproduce/software/bibtex/sextractor.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%% Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sextractor,
       author = {{Bertin}, E. and {Arnouts}, S.},
        title = "{SExtractor: Software for source extraction.}",
      journal = {A\&AS},
     keywords = {METHODS: DATA ANALYSIS, TECHNIQUES: IMAGE PROCESSING, GALAXIES: PHOTOMETRY},
         year = "1996",
        month = "Jun",
       volume = {117},
        pages = {393},
          doi = {10.1051/aas:1996164},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996A&AS..117..393B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sip_tpv.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{sip-tpv,
   author = {{Shupe}, D.~L. and {Laher}, R.~R. and {Storrie-Lombardi}, L. and
	{Surace}, J. and {Grillmair}, C. and {Levitan}, D. and {Sesar}, B.
	},
    title = "{More flexibility in representing geometric distortion in astronomical images}",
     year = 2012,
   journal = {SPIE},
   volume = 8451,
    month = sep,
      eid = {84511M},
    pages = {84511M},
      doi = {10.1117/12.925460},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2012SPIE.8451E..1MS},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/swarp.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{swarp,
   author = {{Bertin}, E. and {Mellier}, Y. and {Radovich}, M. and {Missonnier}, G. and
    {Didelon}, P. and {Morin}, B.},
  journal = {ASPConf},
    title = "{The TERAPIX Pipeline}",
     year = {2002},
   volume = {281},
    pages = {228},
   adsurl = {http://ui.adsabs.harvard.edu/abs/2002ASPC..281..228B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


==> reproduce/software/bibtex/sympy.tex <==
%% Copyright (C) 2019 Raul Infante-Sainz <infantesainz@gmail.com>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@article{sympy,
 title = {SymPy: symbolic computing in Python},
 author = {Meurer, Aaron and Smith, Christopher P. and Paprocki, Mateusz and \v{C}ert\'{i}k, Ond\v{r}ej and Kirpichev, Sergey B. and Rocklin, Matthew and Kumar, AMiT and Ivanov, Sergiu and Moore, Jason K. and Singh, Sartaj and Rathnayake, Thilina and Vig, Sean and Granger, Brian E. and Muller, Richard P. and Bonazzi, Francesco and Gupta, Harsh and Vats, Shivam and Johansson, Fredrik and Pedregosa, Fabian and Curry, Matthew J. and Terrel, Andy R. and Rou\v{c}ka, \v{S}t\v{e}p\'{a}n and Saboo, Ashutosh and Fernando, Isuru and Kulal, Sumith and Cimrman, Robert and Scopatz, Anthony},
 year = 2017,
 month = jan,
 keywords = {Python, Computer algebra system, Symbolics},
 abstract = {
            SymPy is an open source computer algebra system written in pure Python. It is built with a focus on extensibility and ease of use, through both interactive and programmatic applications. These characteristics have led SymPy to become a popular symbolic library for the scientific Python ecosystem. This paper presents the architecture of SymPy, a description of its features, and a discussion of select submodules. The supplementary material provide additional examples and further outline details of the architecture and features of SymPy.
         },
 volume = 3,
 pages = {103},
 journal = {PeerJ CompSci},
 issn = {2376-5992},
 url = {https://doi.org/10.7717/peerj-cs.103},
 doi = {10.7717/peerj-cs.103}
}


==> reproduce/software/bibtex/tides.tex <==
%% Copyright (C) 2019 Mohammad Akhlaghi <mohammad@akhlaghi.org>
%%
%% Copying and distribution of this file, with or without modification,
%% are permitted in any medium without royalty provided the copyright
%% notice and this notice are preserved.  This file is offered as-is,
%% without any warranty.

@ARTICLE{tides,
   author = {{Abad}, A. and {Barrio}, R. and {Belsa}, F. and {Rodriguez}, M},
    title = "{Algorithm 924: TIDES, a Taylor Series Integrator for Differential EquationS}",
  journal = {ACM TOMS},
     year = 2012,
    month = nov,
   volume = 39,
      eid = {5},
    pages = {5:1},
      doi = {10.1145/2382585.2382590},
 keywords = {Taylor series method, automatic differentiation, high precision, numerical integration of ODEs, variational equations},
}

